Transformation & Uncertainty. Some Thoughts on Quantum Probability Theory, Quantum Statistics, and Natural Bundles

This PHD thesis is concerned with uncertainty relations in quantum probability theory, state estimation in quantum stochastics, and natural bundles in differential geometry. After some comments on the nature and necessity of decoherence in open systems and its absence in closed ones, we prove sharp, state-independent inequalities reflecting the Heisenberg principle, the necessity of decoherence and the impossibility of perfect joint measurement. These bounds are used to judge how far a particular measurement is removed from the optimal one. We do this for a qubit interacting with the quantized EM field, continually probed using homodyne detection. We calculate to which extent this joint measurement is optimal. We then propose a two-step strategy to determine the (possibly mixed) state of n identically prepared qubits, and prove that it is asymptotically optimal in a local minimax sense, using `Quantum Local Asymptotic Normality' for qubits. We propose a physical implementation of QLAN, based on interaction with the quantized EM field. In differential geometry, a bundle is called `natural' if diffeomorphisms of the base lift to automorphisms of the bundle. We slightly extend this notion to `infinitesimal naturality', requiring only vector fields (infinitesimal diffeomorphisms) to lift. We classify these bundles. Physical fields that transform under (infinitesimal) space-time transformations must be described in terms of (infinitesimally) natural bundles. All spin structures are infinitesimally natural. Our framework thus encompasses Fermionic fields, for which the notion of a natural bundle is too restrictive. Interestingly, generalized spin structures (e.g. spin-c structures) are not always infinitesimally natural. We classify the ones that are. Depending on the gauge group at hand, this can significantly reduce the number of allowed space-time topologies.

==> defs.tex <==
%%!TEX root = ../proefschrift.tex

%% Document structure
\newcommand{\setsubdir}[1]{%
\def\subdir{#1}%
\graphicspath{\subdir}%
}

\newcommand{\leavesubdir}{%
\makeatletter
\graphicspath{\input@path}
\makeatother
}


\def\subdir{}
\newcommand\Input[1]{\input{\subdir #1}}




%%%% Geen hoofdletters in koptekst bibliografie
\makeatletter
\renewenvironment{thebibliography}[1]
     {\chapter*{\bibname}%
      \@mkboth{\bibname}{\bibname}%
      \list{\@biblabel{\@arabic\c@enumiv}}%
           {\settowidth\labelwidth{\@biblabel{#1}}%
            \leftmargin\labelwidth
            \advance\leftmargin\labelsep
            \@openbib@code
            \usecounter{enumiv}%
            \let\p@enumiv\@empty
            \renewcommand\theenumiv{\@arabic\c@enumiv}}%
      \sloppy
      \clubpenalty4000
      \@clubpenalty \clubpenalty
      \widowpenalty4000%
      \sfcode`\.\@m}
     {\def\@noitemerr
       {\@latex@warning{Empty `thebibliography' environment}}%
      \endlist}
\makeatother

% Voor appendix in hoofdstuk 6
\makeatletter
\def\@Alphminseven#1{\ifcase#1\or A\or B\or C\or D\or E\or F\or G\or A\or B\or J\or K\or L\or M\or N\or O\or P\or Q\or R\or S\or T\or U\or V\or W\or X\or Y\or Z\else\@ctrerr\fi}
\def\Alphminseven#1{\expandafter\@Alphminseven\csname c@#1\endcsname}
\makeatother


%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%...
%% Referencing
\def\Fref#1{Figure~\ref{#1}}
\def\eqref#1{(\ref{#1})}
\def\Eref#1{Equation~(\ref{#1})}
\def\Cref#1{Chapter~\ref{#1}}
\def\Sref#1{Section~\ref{#1}}
\def\Aref#1{Algorithm~\ref{#1}}
\def\Tref#1{Theorem~\ref{#1}}
\def\Href#1{Hoofdstuk~\ref{#1}}

%%% Theorems, Lemmas, Propositions and the likes.

\newtheorem{theorem}{Theorem}[chapter]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{basdef}{Definition}[chapter]
%\newtheorem{remark}[theorem]{Remark}
%\newcommand{\basremark}[1]{\noindent{\bf Remark}\quad{#1}\\ \hfill \noindent}
\newcommand{\basremark}[1]
{{$ $}\\[0.5 ex] \noindent{\bf Remark}\quad {#1}\\[0.5 ex] \noindent}
\newcommand{\sketchproof}{\medskip\noindent{\it Sketch of proof.}\quad}
\newcommand{\proof}{\medskip\noindent{\it Proof.} }
%\newcommand{\remark}{\bigbreak\noindent{\bf Remark.} }
\newcommand{\qed}{\penalty10000\hfill$\Box$\par\goodbreak\medskip\noindent}
%\newcommand{\qed}{${}$ $\hfill \square$}
%%



%%% For `Unifying Decoherence and the Heisenberg Principle'.

%% Grieks %%

\newcommand{\s}{\sigma}
\newcommand{\OO}{\Omega}

%%

%% Breuken %%
\newcommand{\half}{{\textstyle \frac{1}{2}}}
\newcommand{\fourth}{{\textstyle \frac{1}{4}}}

%% Kleinere binom (let op: werkt alleen bij dingen van een teken hoog)
%% (Weer doodgemaakt omdat er ook binoms in de tekst staan.)
%\renewcommand{\binom}[2]{\Bigl(\genfrac{}{}{0pt}{}{#1}{#2}\Bigr)}

%% Hoofdletters %%
\newcommand{\BB}[1]{\mathbb{#1}}
\def\NN{{\mathbb N}}
\def\RR{{\mathbb R}}
\def\PP{{\mathbb P}}
\def\EE{{\mathbb E}}
\def\CCCC{{\mathbb C}}

%% Calligrafisch %%

\newcommand{\CA}{\mathcal{A}}
\newcommand{\CB}{\mathcal{B}}
\newcommand{\CC}{\mathcal{C}}
\newcommand{\CF}{\mathcal{F}}
\newcommand{\CH}{\mathcal{H}}
\newcommand{\CK}{\mathcal{K}}
\newcommand{\CL}{\mathcal{L}}
\newcommand{\CN}{\mathcal{N}}
\newcommand{\CS}{\mathcal{S}}
\newcommand{\CT}{\mathcal{T}}
\newcommand{\CZ}{\mathcal{Z}}
%% X Frac%%
%\newcommand{\x}{\hbox{\sfracFont X}}
\newcommand{\x}{\mathfrak{X}}


%% Wiskunde %%
%\def\tr{{\rm tr}\,}
%\def\Col{{\rm Col}}
\newcommand{\basim}{\mathrm{Im}}
\newcommand{\Col}{|\alpha_0|^2 \ketbra{\psi_0} + |\alpha_1|^2 \ketbra{\psi_1}}
\newcommand{\id}{\mathrm{id}}
\newcommand{\spec}{\mathrm{\textbf{Spec}}}
\newcommand{\ten}{\otimes}
\newcommand{\bra}[1]{\langle#1|}
\newcommand{\ket}[1]{|#1\rangle}
\newcommand{\ketbra}[1]{\ket{#1}\bra{#1}}
\newcommand{\inp}[2]{\langle #1\,|\,#2\rangle}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\norms}[1]{\|#1\|^2}
\newcommand{\one}{\mathbf{1}}
\newcommand{\1}{\hbox{$1$\hspace{-.7pt}%
\vrule width .5pt height 2.5mm depth 0mm\hspace{-0.8mm}%
\vrule width 1.2mm height 0.08mm depth 0mm\hspace{-1.2mm}%
\vrule width 0.7mm height 2.5mm depth -2.42mm}\hspace{.9mm}}
\newcommand{\tr}{\mathbf{tr}}
\newcommand{\dec}{\mathbf{dec}}
\newcommand{\up}{\ket{\! \uparrow \,}\bra{\, \uparrow \!}}
\newcommand{\down}{\ket{\! \downarrow \,}\bra{\, \downarrow \!}}
\newcommand{\abs}[1]{|#1|}
\newcommand{\abss}[1]{|#1|^2}
\newcommand{\dt}{\textstyle \frac{d}{dt}}
\newcommand{\ddt}{\textstyle \frac{d^{2}}{dt^2}}

\newcommand{\spgtitel}{\mathrm{Spin}^{G}}
\newcommand{\spg}
{\mathrm{Spin\raisebox{0.16em}{\textsmaller{G}}}\hspace{0.06em}}
\newcommand{\tf}{\widetilde{F}^{+k}(M)}
\newcommand{\tfx}{\widetilde{F}_{x}^{+k}(M)}
\newcommand{\tgln}{\widetilde{\mathrm{GL}}(\mathbb{R}^{n})}
\newcommand{\tsln}{\widetilde{\mathrm{SL}}(\mathbb{R}^{n})}
\newcommand{\sln}{\mathrm{SL}(\mathbb{R}^{n})}
\newcommand{\gln}{\mathrm{GL}(\mathbb{R}^{n})}
\newcommand{\glnp}{\mathrm{GL}^{+}(\mathbb{R}^{n})}
\newcommand{\glnvp}{\mathrm{GL}^{+}(\mathbb{R}^{4})}
\newcommand{\tdiff}{\widetilde{\mathrm{Diff}}{}^{0}(M)}
\newcommand{\tglnvp}{\widetilde{\mathrm{GL}}{}^{+}(\mathbb{R}^{4})}
\newcommand{\tglnp}{\widetilde{\mathrm{GL}}{}^{+}(\mathbb{R}^{n})}
\newcommand{\lsln}{\mathfrak{sl}(\mathbb{R}^{n})}
\newcommand{\lgln}{\mathfrak{gl}(\mathbb{R}^{n})}
\newcommand{\lsoe}{\mathfrak{so}(\eta)}
\newcommand{\pr}{\pi}
\newcommand{\dg}{\mathrm{dim}(\mathfrak{g})}
\newcommand{\mdiv}{\mathrm{Div}}
\newcommand{\del}{\partial}
\newcommand{\supp}{\mathrm{Supp}}
\newcommand{\vecn}{\mathrm{Vec}_{n}}
\newcommand{\pp}{\mathbb{P}_{\psi}}
\newcommand{\var}{\mathbb{V}\mathrm{ar}}
\newcommand{\vexp}{e}
\newcommand{\vol}{\mathrm{vol}}

%\def\M#1#2{\inp{\ph\ten#1}{\bigl(U^*(\one\ten#2)U\bigr)\ph\ten#1}}

%\def\inp#1#2{\langle#1,#2\rangle}
%\def\bra#1{\langle#1|}
%\def\ket#1{|#1\rangle}
%\def\ketbra#1{|#1\rangle\langle#1|}



%% Mijnfiguur %%

\newcounter{figuur}
\newcommand{\fig}{\refstepcounter{figuur}\textsc{Fig}.\,\arabic{figuur}: }
\newcounter{tempfig}
%%


%%%%% ITISC %%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%% ALLGEMEINES UND FONTS  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\def\square{{\vcenter{\vbox{\hrule height.4pt \hbox{\vrule width.4pt 
%height1.45ex \kern1.45ex \vrule width.4pt}
%\hrule height.4pt}}}}

%\def\qed{\penalty10000\hfill$\square$\par\goodbreak\medskip}
 
%%%%%%%%%%%%%% SYMBOLE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\def\li#1{\lim_{#1\to\infty}}
%\def\soi#1{\sum_{#1=1}^\infty}
%\def\szi#1{\sum_{#1=0}^\infty}
%\def\tuple#1_#2{#1_1,#1_2,\ldots,#1_{#2}}
%\def\tup#1_#2{#1_1,\ldots,#1_{#2}}
%\def\set#1#2{\{#1\;|\;#2\}}

%\def\implies{\Longrightarrow}
%\def\Implies{\quad\Longrightarrow\quad}
%\def\bar#1{{\overline{#1}}}


%% Luc's `theorem' en `definitie' %%
%\newtheoremstyle{mydefi}% name
%  {15pt}%      Space above
%  {15pt}%      Space below
%  {}%         Body font
%  {}%         Indent amount (empty = no indent, \parindent = para indent)
%  {\bfseries}% Thm head font
%  {:}%        Punctuation after thm head
%  {.5em}%     Space after thm head: " " = normal interword space;
%        %       \newline = linebreak
%  {}%         Thm head spec (can be left empty, meaning `normal')
%\newtheoremstyle{mytheo}% name
%  {15pt}%      Space above
%  {15pt}%      Space below
%  {\slshape}%         Body font
%  {}%         Indent amount (empty = no indent, \parindent = para indent)
%  {\bfseries}% Thm head font
%  {:}%        Punctuation after thm head
%  {.5em}%     Space after thm head: " " = normal interword space;
%        %       \newline = linebreak
%  {}%         Thm head spec (can be left empty, meaning `normal')

%\theoremstyle{mytheo}
%\newtheorem{stel}{Theorem}[section]
%\newtheorem{lem}[stel]{Lemma}

%\theoremstyle{mydefi}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> loadheader.tex <==
%% Roep chaptertag aan met `\thechapter'; \chaptertag{\thechapter}
%% Als `\thechapter' gelijk is aan n, wordt chaptertag het ne element
%% van de lijst.
%% 	STEL HIER DUS DE TAGS IN	
%% Ik doe het zo omdat het anders moeilijk is om de pagina voor een hoofdstuk
%% goed te krijgen.

\newcommand{\chaptertag}[1]{%
\ifthenelse{\equal{#1}{1}}{Introduction}{}%
\ifthenelse{\equal{#1}{2}}{Background}{}%
\ifthenelse{\equal{#1}{3}}{Information Transfer}{}%
\ifthenelse{\equal{#1}{4}}{Decoherence}{}%
\ifthenelse{\equal{#1}{5}}{Optimal Pointers}{}%
\ifthenelse{\equal{#1}{6}}{Optimal Estimation}{}%
\ifthenelse{\equal{#1}{7}}{Bundles}{}%					
}

%%%%%%%%%%%%%%%%%%%%%%% 		Headers		 	%%%%%%%%%%%%%
%...
%%	Herdefinieer `cleardoublepage' zodat de pagina links van een beginnend
%%	hoofdstuk HELEMAAL leeg is.

\makeatletter
\def\cleardoublepage{\clearpage\if@twoside \ifodd\c@page\else
  \hbox{}
  \thispagestyle{empty}
  \newpage
  \if@twocolumn\hbox{}\newpage\fi\fi\fi}
\makeatother

%%
%%	Herdefinieer `plain'
%%

  \fancypagestyle{plain}{%
  \fancyhead{}% kill headers
  \fancyfoot{}% and feet
  \renewcommand{\headrulewidth}{0pt}}% and line

%%
%% Handmatig sturen
%%

\newcommand{\handmatigekoptekst}[1]{%
\pagestyle{fancy}%
\fancyhead{}%clear options
\fancyfoot{}%clear options
%% Nu, op even pagina's, "112   `#1'" in TEXTSC
\fancyhead[LE]{\thepage}%
\fancyhead[CE]{\textsc{#1}}%
%% Op oneven pagina's "      113" 
\fancyhead[RO]{\thepage}%
%% Geen voet
\renewcommand{\headrulewidth}{0pt}
%% Geen streep
\renewcommand{\footrulewidth}{0pt}
}
 %% Maak de plain pagina's dood. Geen pagenumber bij nieuw hoofdstuk.

%%
%% Koptekst voor chapters %% 
%%
%TJ \newcommand{\hoofdstukkoptekst}
%TJ {
 \pagestyle{fancy}
 \fancyhead{}%clear options
 \fancyfoot{}%clear options
 %% Nu, op even pagina's, "112   Chapter 3. #1" in TEXTSC
 \fancyhead[LE]{\thepage}
 \fancyhead[CE]{\textsc{\chaptername \, \thechapter. \chaptertag{\thechapter}}}
 %% Op oneven pagina's "1.5  Introduction" in TEXTSC
 %\renewcommand{\sectionmark}[1]{\markright{\thesection\  \textsc{#1}}}
 %\fancyhead[LO]{\rightmark}
 \fancyhead[RO]{\thepage}
 %% Geen voet
 \renewcommand{\headrulewidth}{0pt}
 %% Geen streep
 \renewcommand{\footrulewidth}{0pt}
 %% Maak de plain pagina's dood. Geen pagenumber bij nieuw hoofdstuk.
%TJ }

%%

